Exploring the Potential of Generative AI for the World Wide Web

Generative Artificial Intelligence (AI) is a cutting-edge technology capable of producing text, images, and various media content leveraging generative models and user prompts. Between 2022 and 2023, generative AI surged in popularity with a plethora of applications spanning from AI-powered movies to chatbots. In this paper, we delve into the potential of generative AI within the realm of the World Wide Web, specifically focusing on image generation. Web developers already harness generative AI to help crafting text and images, while Web browsers might use it in the future to locally generate images for tasks like repairing broken webpages, conserving bandwidth, and enhancing privacy. To explore this research area, we have developed WebDiffusion, a tool that allows to simulate a Web powered by stable diffusion, a popular text-to-image model, from both a client and server perspective. WebDiffusion further supports crowdsourcing of user opinions, which we use to evaluate the quality and accuracy of 409 AI-generated images sourced from 60 webpages. Our findings suggest that generative AI is already capable of producing pertinent and high-quality Web images, even without requiring Web designers to manually input prompts, just by leveraging contextual information available within the webpages. However, we acknowledge that direct in-browser image generation remains a challenge, as only highly powerful GPUs, such as the A40 and A100, can (partially) compete with classic image downloads. Nevertheless, this approach could be valuable for a subset of the images, for example when fixing broken webpages or handling highly private content.

==> sections/discussion-notes.tex <==
\vspace{0.05in}
\noindent
\textbf{Performance Optimizations:} This paper has highlighted two areas of improvements when applying text-to-image generation to the Web. First, the \textit{quality} of images involving human subjects, notably face and hands deformation, and second the \textit{speed} at which images are generated. Quality and speed are directly related to the number of iterations; in this paper we settle for a constant number of inference steps (\numiter) for fairness between images of different webpages (see Section~\ref{sec:meth:stable}). An interesting research area is to explore stable diffusion's parameters as a function of the textual prompt content.

%JH -- please check if this works?
We experimented with modifying the seed and the number of inference steps of the model until the sampled output was artefact-free and acceptable. However, such a detailed sampling process could not be upscaled automatically given the difficulty in detecting the artefact or fit of the generated images without human intervention. Nonetheless, we concluded that dynamic parameters –– modifying the seed and iterations parameters depending on image content –– could also be a viable method to optimize the performance of \tool and reduce the artefacts in its output.
%JH -- feels like things start falling apart at the end here

%Another possible solution, which takes into account both the prevention of unwanted artefacts and improving computation speeds, is the construction of dynamic parameters for the number of iterations and the seed for the sampling. Either manually or automatically adjusting the iterations before output based on the content of the image could help avoid needless computations. In addition, upon finding a sampled output that best captures the original image, content providers could assign specific seeds to ensure that artefacts are either not present or the images are realistic.

Indeed, we observed that stable diffusion often produces artefacts when generating images of faces and hands even with a large number of iterations (> 100, increasing the image generation time to above 15 seconds), especially when there are more than one subject in the produced image. We also noted that stable diffusion is capable of generating convincing and realistic portrayals of landscapes even with a low number of iterations (as low as 10, which can generate an image within a second). These results may be attributed to the fact that the stable diffusion model was trained on the LAION Aesthetic dataset~\cite{LAION_aesthetic}, comprised of numerous paintings and artistic photography, meaning that the training set would need to be diversified in order to produce more realistic, artefact-free results. Alternatively, one could consider extending \tool to other text-to-image generation models. For example, the GFPGAN model is a popular method that addresses the issue of distorted faces. This model helps restore faces in samples and improves the overall realistic quality of the generated image~\cite{gfpgan}.

Another area for optimization is the computation speed of the stable diffusion model. As stable diffusion is still a recent topic of exploration, there are constant developments in the areas of its computational efficiency and speed. One example of this is switching a large portion of the cross attention operations within the sampling process to FLASH attention, which can increase computation speeds by nearly 50 percent while decreasing VRAM usage ~\cite{flash_paper, flash_attention}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{0.05in}
\noindent
\textbf{Privacy-Preserving Advertisement:} On-line advertisement heavily relies on tracking, where user profiles and information are auctioned, in real time, to tens or hundred of ad networks. The privacy concerns of such approach are clear, and they have motivated the rise of adblockers and private models of advertising like the one offered by the Brave browser~\cite{brave}. In Brave, user profiles are local and never leave the browser. Still, network requests are needed to fetch the ads to be shown, \eg GET an image containing a sport car for a car enthusiast profile. These requests are answered in the cloud, where some potential privacy leak is possible. Local ads generation remove even the slightest privacy leak from the, already private, Brave model. 

\vspace{0.05in}
\noindent
\textbf{Broken URLs:} The Web is an ever-growing ecosystem and, as such, many webpages are often unreachable or miss some important content. The Wayback Machine~\cite{wayback} is an interesting approach to deal with broken pages, since it currently offers 751 billion saved webpages. Our client-based approach can help in such scenarios, where missing images can be recovered by mean of the contextual information available in the page. 
